Auto-Encoding Goodness of Fit

We develop a new type of generative autoencoder called the Goodness-of-Fit Autoencoder (GoFAE), which incorporates GoF tests at two levels. At the minibatch level, it uses GoF test statistics as regularization objectives. At a more global level, it selects a regularization coefficient based on higher criticism, i.e., a test on the uniformity of the local GoF p-values. We justify the use of GoF tests by providing a relaxed $L_2$-Wasserstein bound on the distance between the latent distribution and a distribution class. We prove that optimization based on these tests can be done with stochastic gradient descent on a compact Riemannian manifold. Empirically, we show that our higher criticism parameter selection procedure balances reconstruction and generation using mutual information and uniformity of p-values respectively. Finally, we show that GoFAE achieves comparable FID scores and mean squared errors with competing deep generative models while retaining statistical indistinguishability from Gaussian in the latent space based on a variety of hypothesis tests.

==> additional-experiment.tex <==
\section{Additional Experiments}
%%%%% PLOTS, FIGURES and TABLES
In this section, we are able to visually assess the quality of our GoFAE models. To be considered successful, when a ``good" regularization coefficient $\lambda > 0$ is selected, the model should (i) fail to reject $\mathcal{H}_0$ at an $\alpha$-level chosen a-priori (close to normal but not overly so), (ii) accurately reconstruct the input, and finally (iii) be able to generate samples which are both qualitatively and quantitatively convincing. 

Section E.3.1. contains the figures produced by training a variety of GoFAEs on the CelebA dataset with a latent space dimension of 64. Figure \ref{fig:celeba-recon-faces} depicts the reconstructed faces from a variety of models. In Table 1 in the main paper, we evaluated reconstruction quality with mean-squared error and the Frechet-Inception Distance (FID). The GoFAE models produced some of the lowest MSE, reconstruction FID which agreed visually when compared against the ground truth and competitor models. Figure \ref{fig:celeba-gen-faces} contains faces generated from the model. The GoFAE models again produced competitive FID scores, with GoFAE-SF producing the lowest (best) of the group.

There are several things to note from the information contained in Table \ref{tab:celeba-lines-sw-sf} and Table \ref{tab:celeba-lines-cvm-ks}. The first row shows the normality behaviour as a function of $\text{log}(\lambda)$. As $\lambda$ increases the models are producing aggregated posteriors that are appearing increasingly indistinguishable from normal. However, beyond a certain point, the encoding no longer appears normal, GoFAE-SW clearly depicts this occurring in Table (S2a-SW). The row (b) tracks the average $p$-value produced on a test set while training with a particular GoF test statistic. Larger $\lambda$ can easily be seen to focus more on normality as the p-values tend to start at high levels and stay. The reconstruction error in row (c) tends to converge quickly. 

We find it particularly interesting how in the plots of $\text{log}(\lambda)$ vs KS $p$-value, once the average KS uniformity peaks, the mutual information falls rapidly after. This clearly illustrates the relationship posited in the experiments section where the model prioritizes posterior matching.

Similar plots for MNIST can be seen in section E.3.2. with the quantitative information regarding reconstruction error, reconstruction FID and generation FID in Table \ref{tab:mnist-fid-tab}. Once again, the GoFAE models produce overall lower MSE than competitor models, while maintaining competitive generation FID scores. 

\subsection{Details on Experiments}
We trained GoFAEs on the MNIST \cite{lecun1998}, CelebA \cite{liu2015}, and Cifar-10 \cite{krizhevsky2009learning}.
\subsubsection{MNIST}
The MNIST dataset was re-scaled to the unit interval. Training proceeded for 50 epochs using mini-batches of size 128. 
%The CelebA dataset was pre-processed following the same procedure in \cite{tolstikhin2017}, first a 140x140 center crop is taken and the image is resized to $64 \times 64$ resolution. 
To keep comparisons the same, we adopted a common architecture among all methods. The section above contains the architecture used for which dataset. Competitor models include $\beta$-VAE \cite{higgins2016}, VAE \cite{kingma2013}, WAE-GAN \cite{tolstikhin2017}, VAE with learned $\gamma$ \cite{dai2019diagnosing}, 2-Stage VAE \cite{dai2019diagnosing}, and AE \cite{bengio2013representation}. Both VAE and $\beta$-VAE had an initial learning rate of $1e-4$, while VAE with learnable $\gamma$ used $1e-3$. 

For our models, Adam optimizer \cite{kingma2014} was used for the encoder (learning rate $3e-3$, $\beta = (0.5, 0.999)$) and decoder (learning rate $3e-3$, $\beta = (0.5, 0.999)$). Riemannian SGD, learning rate 5e-3, was used to constrain $\bm{\Theta}$ to the Stiefel manifold using a one cycle learning rate scheduler with max learning rate as 1e-3. Singular value decomposition was used for retracting $\bm{\Theta}$ back to $\mathcal{M}$ after an update. Our models were trained on a high performance cluster using V100, RTX and GTX graphics cards.


\subsubsection{CelebA}
%The dataset was processed by taking $140 \times 140$ center crops of the images followed by resizing to $64 \times 64$. The dimension of the 
The CelebA dataset was pre-processed following the same procedure in \cite{tolstikhin2017}, first a 140x140 center crop is taken and the image is resized to $64 \times 64$ resolution. 
For the VAE, the Adam optimizer was used with a learning rate of $1e-4$, and $\beta_1=0.5$ and $\beta_2=0.999$. The $\beta$-VAE, the Adam optimizer used with a learning rate of $1e-4$, $\beta_1=0.5$, and $\beta_2=0.999$. The VAE with learnable $\gamma$, the Adam optimizer was used with a learning rate of $1e-3$, $\beta_1=0.5$, and $\beta_2=0.999$. For the WAE-GAN, the Adam optimizer was used where the encoder and decoder parameters has an initial learning rate of $3e-4$ and the discriminator was set to $1e-3$ with $\beta_1=0.5$, $\beta_2=0.999$. For the two-stage VAE, we used the trained VAE with learned gamma as stage one. A second VAE was trained using the $\mu, \sigma$ from the first stage as inputs. The architecture was a three layer dense net with relu activations, and the decoder was the inverse, with a final linear layer.

For our method, which had two components for the encoder, as visualized in Figure (3a) in the main paper. The first component of the encoder used the Adam optimizer with learning rate set to $3e-3$ and $\beta_1=0.5$ and $\beta_2=0.999$. The decoder also used Adam, with same learning rates and hyper parameters. The dense layer of the encoding processes is parameterized by $\bm{\Theta}$, an element of the Steifel manifold $\mathcal{M}$, and is trained with Riemannian SGD with a learning rate of $5e-3$ while making use of the 1-Cycle learning rate scheduler with a maximum learning rate of $1e-3$.

As our methods require projection, a $64 \times 64$ dimensional orthonormal basis is sampled and used to project the encoded data.


% %All methods use the same decoding architecture.

% \iffalse
% All models use mini-batches of size 128.

% \subsubsection{MNIST}


% Trained for 50 epochs.

% Our models:

% Competitor models:



% \subsubsection{CelebA}
% The dataset was processed by taking $140 \times 140$ center crops of the images followed by resizing to $64 \times 64$. The dimension of the 

% For the VAE, the Adam optimizer was used with a learning rate of $1e-4$, and $\beta_1=0.5$ and $\beta_2=0.999$. The $\beta$-VAE, the Adam optimizer used with a learning rate of $1e-4$, $\beta_1=0.5$, and $\beta_2=0.999$. The VAE with learnable $\gamma$, the Adam optimizer was used with a learning rate of $1e-3$, $\beta_1=0.5$, and $\beta_2=0.999$. For the WAE-GAN, the Adam optimizer was used where the encoder and decoder parameters has an initial learning rate of $3e-4$ and the discriminator was set to $1e-3$ with $\beta_1=0.5$, $\beta_2=0.999$. For the two-stage VAE, we used the trained VAE with learned gamma as stage one. A second VAE was trained using the $\mu, \sigma$ from the first stage as inputs. The architecture was a three layer dense net with relu activations, and the decoder was the inverse, with a final linear layer.

% For our method, which had two components for the encoder, as visualized in Figure (3a) in the main paper. The first component of the encoder used the Adam optimizer with learning rate set to $3e-3$ and $\beta_1=0.5$ and $\beta_2=0.999$. The decoder also used Adam, with same learning rates and hyper parameters. The dense layer of the encoding processes is parameterized by $\bm{\Theta}$, an element of the Steifel manifold $\mathcal{M}$, and is trained with Riemannian SGD with a learning rate of $5e-3$ while making use of the 1-Cycle learning rate scheduler with a maximum learning rate of $1e-3$.

% As our methods require projection, a $64 \times 64$ dimensional orthonormal basis is sampled and used to project the encoded data.




% \subsubsection{Cifar10}
% Trained for 200 epochs.

% Our models:

% Competitor models:
% \fi

\subsection{MNIST}
%Inception score has been replaced with FID in Table \ref{tab:mnist-fid-tab}.
%The encoder/decoder architectures followed are described in Appendix Section C. We specified a 10-dimensional code layer  


%We followed the original authors \cite{heusel2017} suggestion for computing the necessary statistics. The FID score produced from the true and generated statistics are what is in the table. As always, lower is preferred.

\begin{table*}[!htb]
\captionsetup{type=table} %% tell latex to change to table
\caption{%Apendix Table 2 update: 
FID \cite{heusel2017} scores for reconstruction and samples ( mean (std) ) with p-values from the higher criticism evaluation.}\label{tab:mnist-fid-tab}
%The first row is Kolmogorov-Smirnov uniform test for the p-values, and the second row (SW, CVM, KS, HZ) are the normality tests used to compute the p-values.}\label{tab:maintab}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|l|ll|lllll}
\hline
\multirow{2}{*}{Algorithm} & \multirow{2}{*}{MSE $\downarrow$} & \multicolumn{2}{c|}{FID Score $\downarrow$} & \multicolumn{5}{c}{Kolmogorov-Smirnov Uniformity Test}              \\ \cline{3-9} 
                           &                                   & Gen.                 & Recon.                   & SW          & SF          & CVM         & KS          & EP          \\ \hline
AE-Baseline                & 7.66                              &    107.15     &  14.37       & 0.0 (0.0)   & 0.0 (0.0)   & 0.0 (0.0)   & 0.0 (0.0)   & 0.0 (0.0)   \\
VAE                        & 13.99                             &   21.29      &   15.78    & 0.18 (0.18) & 0.42 (0.30) & 0.07 (0.12) & 0.14 (0.18) & 0.03 (0.06) \\
$\beta(2)$-VAE             & 20.98                             &    28.95     &    19.42     & 0.38 (0.31) & 0.29 (0.26) & 0.41 (0.29) & 0.45 (0.31) & 0.24 (0.25) \\
C-$\beta$-VAE              & 20.94                             &    25.55     &    19.22     & 0.48 (0.30) & 0.37 (0.28) & 0.29 (0.26) & 0.42 (0.31) & 0.19 (0.19) \\
WAE-GAN                    & 9.49                              &   22.33      &   \textbf{13.51}   & 0.07 (0.12) & 0.49 (0.29) & 0.09 (0.15) & 0.11 (0.12) & 0.06 (0.12) \\ \hline
GoFAE-SW                   & 7.16                              &   21.99      &     14.52   & 0.11 (0.16) & 0.48 (0.23) & 0.06 (0.12) & 0.17 (0.24) & 0.03 (0.05) \\
GoFAE-SF                   & \textbf{7.08}                     &  26.89       &    14.53     & 0.0 (0.0)   & 0.26 (0.27) & 0.0 (0.0)   & 0.0 (0.0)   & 0.0 (0.0)   \\
GoFAE-CVM                  & 7.67                              &    \textbf{19.08}     &    14.82     & 0.14 (0.18) & 0.46 (0.28) & 0.14 (0.22) & 0.12 (0.21) & 0.05 (0.15) \\
GoFAE-EP                   & 7.54                              &     22.36    &  14.95     & 0.25 (0.27) & 0.44 (0.28) & 0.12 (0.23) & 0.17 (0.20) & 0.05 (0.08) \\ \hline
\end{tabular}
}
\end{table*}
%We can see that the GoF test regularizers for MNIST perform reasonably well, with small MSE on test set


\begin{figure}[H]
    \centering
    \includegraphics[width = \textwidth]{figs/NIPS22_rebuttal_plots/mnist/SW_MI_CN.png}
    \caption{Effects of $\lambda$. We evaluated the uniformaty KS test (blue), mutual information (red), log conditional number (green) and reconstruction (black) under different $\lambda$ for GoFAE-SW.}
    \label{fig:mnist-sw-mi-cn}
\end{figure}
%In Figure (\ref{fig:mnist-sw-mi-cn})


\newpage
\subsection{Additional Plots}
In this section, we included more experiment results for GoFAE and comparison models. 

\subsubsection{celebA}
Figure \ref{fig:celeba-recon-faces} and Figure \ref{fig:celeba-gen-faces} provided reconstructed images and random generated samples from each model for CelebA dataset. Table \ref{tab:celeba-lines-sw-sf} and \ref{tab:celeba-lines-cvm-ks} illustrated in detail the effects of $\lambda$ on KS uniformity test, corresponding p-value, reconstruction error, and test statistics for GoFAE-SW, GoFAE-SF, GoFAE-CVM and GoFAE-KS, respectively. As discussed in Section 5 and Table 1 in the main paper, the GoFAE models are competitive in construction and generation while the statistical indistinguishability from Gaussian is retained. 
% celebA reconstruction
\newpage
\graphicspath{{figs/NIPS22_rebuttal_plots/celeba/}}
\begin{figure}[H]\centering
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./ae/ground_truth.png}\caption{Ground truth}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./ae/epoch_50_recon.png}\caption{AE}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./vae/epoch_50_recon.png}\caption{VAE (fixed $\gamma$)}
\end{subfigure}     

\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./vaeLG/epoch_50_recon.png}\caption{VAE (learned $\gamma$)}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./bvae/10.0/epoch_50_recon.png}\caption{$\beta(10)$-VAE}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./waegan/epoch_50_recon.png}\caption{WAE-GAN}
\end{subfigure}    

% \begin{subfigure}[b]{0.32\textwidth}
% \includegraphics[width=\textwidth]{./cbvae/5/25/epoch_50_recon.png}\caption{C-$\beta$-VAE}
% \end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./twostagevae/epoch_50_recon.png}\caption{2-Stage VAE}
\end{subfigure} \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./sw/epoch_50_recon.png}\caption{GoFAE-SW}
\end{subfigure} \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./sf/epoch_50_recon.png}\caption{GoFAE-SF}
\end{subfigure}     

\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./cvm/epoch_50_recon.png}\caption{GoFAE-CVM}
\end{subfigure}    
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./ks/epoch_50_recon.png}\caption{GoFAE-KS} 
\end{subfigure}    
\caption{Comparison of reconstruction between competing methods: (b) AE, (c) VAE (fixed $\gamma$), (d) VAE (learned $\gamma$), (e) $\beta$-VAE ($\beta = 10$), (f) WAE-GAN, (g) 2-Stage VAE, and our framework: (h) GoFAE-SW, (i) GoFAE-SF, (j) GoFAE-CVM, (k) GoFAE-KS with CelebA.}\label{fig:celeba-recon-faces}
\end{figure}


% celebA generation
\graphicspath{{figs/NIPS22_rebuttal_plots/celeba/}}
\begin{figure}[H]\centering
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./ae/ground_truth.png}\caption{Ground truth}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./ae/epoch_50_gen.png}\caption{AE}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./vae/epoch_50_gen.png}\caption{VAE (fixed $\gamma$)}
\end{subfigure}     

\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./vaeLG/epoch_50_gen.png}\caption{VAE (learned $\gamma$)}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./bvae/10.0/epoch_50_gen.png}\caption{$\beta(10)$-VAE}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./waegan/epoch_50_gen.png}\caption{WAE-GAN}
\end{subfigure}    

% \begin{subfigure}[b]{0.32\textwidth}
% \includegraphics[width=\textwidth]{./cbvae/5/25/epoch_50_gen.png}\caption{C-$\beta$-VAE}
% \end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./twostagevae/epoch_50_gen.png}\caption{2-Stage VAE}
\end{subfigure} \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./sw/epoch_50_gen.png}\caption{GoFAE-SW}
\end{subfigure} \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./sf/epoch_50_gen.png}\caption{GoFAE-SF}
\end{subfigure}   

\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./cvm/epoch_50_gen.png}\caption{GoFAE-CVM}
\end{subfigure}     
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./ks/epoch_50_gen.png}\caption{GoFAE-KS} 
\end{subfigure}    
\caption{Comparison of generated samples between competing methods: (b) AE, (c) VAE (fixed $\gamma$), (d) VAE (learned $\gamma$), (e) $\beta$-VAE ($\beta = 10$), (f) WAE-GAN, (g) 2-Stage VAE, and our framework: (h) GoFAE-SW, (i) GoFAE-SF, (j) GoFAE-CVM, (k) GoFAE-KS with CelebA.}\label{fig:celeba-gen-faces}
\end{figure}

% celebA line plots SW and SF
\graphicspath{{figs/NIPS22_rebuttal_plots/celeba/}}
\begin{table}[H]
\captionsetup{type=table} %% tell latex to change to table
\caption{The effects of $\lambda$ with GoFAE-SW (left) and GoFAE-SF (right) for CelebA. From top to bottom, we have: (a) the normality of GoFAE mini-batch encodings using 30 repetitions of Algorithm 1 for different $\lambda$. (b) $p$-value changing from epoch 1-50 under varying $\lambda$. (c) Reconstruction error on the testing set with different $\lambda$. (d) Test statistics value on the testing set with different $\lambda$. }\label{tab:celeba-lines-sw-sf}
\centering
\setlength\tabcolsep{3pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{cM{50mm}M{50mm}}
\toprule
  & GoFAE-SW & GoFAE-SF \\
\midrule
%\rotatebox[origin=c]{90}{plot1} &
(a) & 
\includegraphics[width=14em]{./sw/plots/pval_vs_mi.png} & 
\includegraphics[width=14em]{./sf/plots/pval_vs_mi.png} \\
%\rotatebox[origin=c]{90}{plot2} &
(b) &
\includegraphics[width=14em]{./sw/plots/test_pval_lambda.png} & 
\includegraphics[width=14em]{./sf/plots/test_pval_lambda.png} \\
%\rotatebox[origin=c]{90}{plot3} &
(c) &
\includegraphics[width=14em]{./sw/plots/test_recon_lambda.png} & 
\includegraphics[width=14em]{./sf/plots/test_recon_lambda.png} \\
%\rotatebox[origin=c]{90}{plot4} & 
(d) &
\includegraphics[width=14em]{./sw/plots/test_tstat_lambda.png} & 
\includegraphics[width=14em]{./sf/plots/test_tstat_lambda.png} \\
\bottomrule
\end{tabular}}
\end{table}



% celebA line plots CVM and KS
\graphicspath{{figs/NIPS22_rebuttal_plots/celeba/}}
\begin{table}[H]
\captionsetup{type=table} %% tell latex to change to table
\caption{The effects of $\lambda$ with GoFAE-CVM (left) and GoFAE-KS (right) for CelebA. From top to bottom, we have: (a) the normality of GoFAE mini-batch encodings using 30 repetitions of Algorithm 1 for different $\lambda$. (b) $p$-value changing from epoch 1-50 under varying $\lambda$. (c) Reconstruction error on the testing set with different $\lambda$. (d) Test statistics value on the testing set with different $\lambda$. }\label{tab:celeba-lines-cvm-ks}
\centering
\setlength\tabcolsep{2pt}
\resizebox{\textwidth}{!}{
%\begin{tabular}{l*2{C}@{}}
\begin{tabular}{cM{50mm}M{50mm}}
\toprule
   & CVM & KS \\
\midrule
(a) & 
\includegraphics[width=14em]{./cvm/plots/pval_vs_mi.png} & 
\includegraphics[width=14em]{./ks/plots/pval_vs_mi.png} \\
(b) & 
\includegraphics[width=14em]{./cvm/plots/test_pval_lambda.png} & 
\includegraphics[width=14em]{./ks/plots/test_pval_lambda.png} \\
(c) & 
\includegraphics[width=14em]{./cvm/plots/test_recon_lambda.png} & 
\includegraphics[width=14em]{./ks/plots/test_recon_lambda.png} \\
(d) & 
\includegraphics[width=14em]{./cvm/plots/test_tstat_lambda.png} & 
\includegraphics[width=14em]{./ks/plots/test_tstat_lambda.png} \\
\bottomrule
\end{tabular}
}
\end{table}


\subsubsection{MNIST}
In this section, we included additional reconstruction and generation samples in Figure \ref{fig:mnist-recon-fig} and Figure \ref{fig:mnist-GEN-fig}. Table \ref{tab:mnist-lines-sw-sf} and \ref{tab:mnist-lines-cvm-ks} demonstrated the effects of $\lambda$ on KS uniformity test, corresponding p-value, reconstruction error, and test statistics for GoFAE-SW, GoFAE-SF, GoFAE-CVM and GoFAE-KS, respectively. The experiments on MNIST reach the same conclusion as in the CelebA, that our GoFAE methods is competitive in both reconstruction and generation. 
\newpage

% \begin{table*}[!htb]
% \captionsetup{type=table} %% tell latex to change to table
% \caption{Apendix Table 2 update: FID scores for reconstruction and samples ( mean (std) ) with p-values from the higher criticism evaluation.}\label{tab:mnist-fid-tab}
% %The first row is Kolmogorov-Smirnov uniform test for the p-values, and the second row (SW, CVM, KS, HZ) are the normality tests used to compute the p-values.}\label{tab:maintab}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|l|ll|lllll}
% \hline
% \multirow{2}{*}{Algorithm} & \multirow{2}{*}{MSE $\downarrow$} & \multicolumn{2}{c|}{FID Score $\downarrow$} & \multicolumn{5}{c}{Kolmogorov-Smirnov Uniformity Test}              \\ \cline{3-9} 
%                           &                                   & Recon.                 & Gen.                   & SW          & SF          & CVM         & KS          & EP          \\ \hline
% AE-Baseline                & 7.66                              &         &         & 0.0 (0.0)   & 0.0 (0.0)   & 0.0 (0.0)   & 0.0 (0.0)   & 0.0 (0.0)   \\
% VAE                        & 13.99                             &         &       & 0.18 (0.18) & 0.42 (0.30) & 0.07 (0.12) & 0.14 (0.18) & 0.03 (0.06) \\
% $\beta(2)$-VAE             & 20.98                             &         &         & 0.38 (0.31) & 0.29 (0.26) & 0.41 (0.29) & 0.45 (0.31) & 0.24 (0.25) \\
% C-$\beta$-VAE              & 20.94                             &         &         & 0.48 (0.30) & 0.37 (0.28) & 0.29 (0.26) & 0.42 (0.31) & 0.19 (0.19) \\
% WAE-GAN                    & 9.49                              &         &      & 0.07 (0.12) & 0.49 (0.29) & 0.09 (0.15) & 0.11 (0.12) & 0.06 (0.12) \\ \hline
% GoFAE-SW                   & 7.16                              &         &        & 0.11 (0.16) & 0.48 (0.23) & 0.06 (0.12) & 0.17 (0.24) & 0.03 (0.05) \\
% GoFAE-SF                   & \textbf{7.08}                     &         &         & 0.0 (0.0)   & 0.26 (0.27) & 0.0 (0.0)   & 0.0 (0.0)   & 0.0 (0.0)   \\
% GoFAE-CVM                  & 7.67                              &         &         & 0.14 (0.18) & 0.46 (0.28) & 0.14 (0.22) & 0.12 (0.21) & 0.05 (0.15) \\
% GoFAE-EP                   & 7.54                              &         &       & 0.25 (0.27) & 0.44 (0.28) & 0.12 (0.23) & 0.17 (0.20) & 0.05 (0.08) \\ \hline
% \end{tabular}
% }
% \end{table*}

\graphicspath{{figs/NIPS22_rebuttal_plots/mnist/}}
\begin{figure}[H]\centering
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./ae/ground_truth.png}\caption{Ground truth}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./ae/recon_epoch_50.png}\caption{AE}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./vae/epoch_50_recon.png}
\caption{VAE}
\end{subfigure}   

\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./bvae/recon_epoch_50.png}\caption{$\beta(2)$-VAE}% (fixed $\gamma$)}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./cbvae/recon_epoch_50.png}\caption{C-$\beta$-VAE}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./waegan/epoch_50_recon.png}\caption{WAE-GAN}
\end{subfigure}    
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./sw/epoch_50_recon.png}\caption{GoFAE-SW}
\end{subfigure} \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./sf/epoch_50_recon.png}\caption{GoFAE-SF}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./ep1/epoch_50_recon.png}\caption{GoFAE-EP}
\end{subfigure}     

\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./cvm/epoch_50_recon.png}\caption{GoFAE-CVM}
\end{subfigure}
\caption{Comparison of reconstruction between competing methods (b) AE, (c) VAE, (d) $\beta$-VAE ($\beta = 2$), (e) C-$\beta$-VAE, (f) WAE-GAN, and our framework: (g) GoFAE-SW, (h) GoFAE-SF, (i) GoFAE-EP, (j) GoFAE-CVM with MNIST.}\label{fig:mnist-recon-fig}
\end{figure}

% mnist generation
\graphicspath{{figs/NIPS22_rebuttal_plots/mnist/}}
\begin{figure}[H]\centering
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./ae/ground_truth.png}\caption{Ground truth}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./ae/samp_epoch_50.png}\caption{AE}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./vae/epoch_50_gen.png}
\caption{VAE}
\end{subfigure}   

\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./bvae/samp_epoch_50.png}\caption{$\beta(2)$-VAE}% (fixed $\gamma$)}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./cbvae/samp_epoch_50.png}\caption{C-$\beta$-VAE}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./waegan/epoch_50_gen.png}\caption{WAE-GAN}
\end{subfigure}    


\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./sw/epoch_50_gen.png}\caption{GoFAE-SW}
\end{subfigure} \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./sf/epoch_50_gen.png}\caption{GoFAE-SF}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./ep1/epoch_50_gen.png}\caption{GoFAE-EP}
\end{subfigure}     

\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./cvm/epoch_50_gen.png}\caption{GoFAE-CVM}
\end{subfigure} 
\caption{Comparison of generated samples between competing methods (b) AE, (c) VAE, (d) $\beta$-VAE ($\beta = 2$), (e) C-$\beta$-VAE, (f) WAE-GAN, and our framework: (g) GoFAE-SW, (h) GoFAE-SF, (i) GoFAE-EP, (j) GoFAE-CVM with MNIST.}\label{fig:mnist-GEN-fig}
\end{figure}


% mnist line plots SW SF
\graphicspath{{figs/NIPS22_rebuttal_plots/mnist/}}
\begin{table}[H]
\captionsetup{type=table} %% tell latex to change to table
\caption{The effects of $\lambda$ with GoFAE-SW (left) and GoFAE-SF (right) for MNIST. From top to bottom, we have: (a) $p$-value changing from epoch 1-50 under varying $\lambda$. (b) Reconstruction error on the testing set with different $\lambda$. (c) Test statistics value on the testing set with different $\lambda$. }\label{tab:mnist-lines-sw-sf}
\centering
\setlength\tabcolsep{2pt}
\resizebox{\textwidth}{!}{
%\begin{tabular}{l*2{C}@{}}
\begin{tabular}{cM{50mm}M{50mm}}
\toprule
   & GoFAE-SW & GoFAE-SF \\
\midrule
(a) & 
\includegraphics[width=14em]{./sw/plots/test_pval_lambda.png} & 
\includegraphics[width=14em]{./sf/plots/test_pval_lambda.png} \\
(b) & 
\includegraphics[width=14em]{./sw/plots/test_recon_lambda.png} & 
\includegraphics[width=14em]{./sf/plots/test_recon_lambda.png} \\
(c) & 
\includegraphics[width=14em]{./sw/plots/test_tstat_lambda.png} & 
\includegraphics[width=14em]{./sf/plots/test_tstat_lambda.png} \\
\bottomrule
\end{tabular}
}
\end{table}


\graphicspath{{figs/NIPS22_rebuttal_plots/mnist/}}
\begin{table}[H]
\captionsetup{type=table} %% tell latex to change to table
\caption{The effects of $\lambda$ with GoFAE-CVM (left) and GoFAE-EP (right) for MNIST. From top to bottom, we have: (a) $p$-value changing from epoch 1-50 under varying $\lambda$. (b) Reconstruction error on the testing set with different $\lambda$. (c) Test statistics value on the testing set with different $\lambda$. }\label{tab:mnist-lines-cvm-ks}
\centering
\setlength\tabcolsep{2pt}
\resizebox{\textwidth}{!}{
%\begin{tabular}{l*2{C}@{}}
\begin{tabular}{cM{50mm}M{50mm}}
\toprule
   & GoFAE-CVM & GoFAE-EP    \\
\midrule
(a) & 
\includegraphics[width=14em]{./cvm/plots/test_pval_lambda.png} & 
\includegraphics[width=14em]{./ep1/plots/test_pval_lambda.png} \\
(b) & 
\includegraphics[width=14em]{./cvm/plots/test_recon_lambda.png} & 
\includegraphics[width=14em]{./ep1/plots/test_recon_lambda.png} \\
(c) & 
\includegraphics[width=14em]{./cvm/plots/test_tstat_lambda.png} & 
\includegraphics[width=14em]{./ep1/plots/test_tstat_lambda.png} \\
\bottomrule
\end{tabular}
}
\end{table}

\iffalse
\subsubsection{CIFAR-10}
% table for CIFAR-10 



% reconstruction
\graphicspath{{figs/NIPS22_rebuttal_plots/cifar/}}
\begin{figure}[H]\centering
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./bvae/ground_truth.png}
\caption{Ground truth}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{example-image}%{./ae/epoch_200_recon.png}
\caption{AE}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./vae/epoch_200_recon.png}
\caption{VAE (fixed $\gamma$)}
\end{subfigure}     

\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./vaeLG/epoch_200_recon.png}
\caption{VAE (learned $\gamma$)}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./bvae/epoch_200_recon.png}
\caption{$\beta(10)$-VAE}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./waegan/epoch_200_recon.png}
\caption{WAE-GAN}
\end{subfigure}    

\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{example-image}%{./cbvae/5/25/epoch_50_recon.png}
\caption{CBVAE}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./twostagevae/epoch_last_recon.png}
\caption{2-Stage VAE}
\end{subfigure} \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{example-image}%{./sw/epoch_50_recon.png}
\caption{GoFAE-SW}
\end{subfigure} 

\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{example-image}%{./sf/epoch_50_recon.png}
\caption{GoFAE-SF}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{example-image}%{./cvm/epoch_50_recon.png}
\caption{GoFAE-CVM}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{example-image}%{./ks/epoch_50_recon.png}
\caption{GoFAE-KS} 
\end{subfigure}    
\caption{Comparison of reconstruction between AE, VAE, $\beta$-VAE, WAE-GAN, $2-$Stage VAE and GoFAE.}\label{fig:cifar-recon-imgs}
\end{figure}


% cifar generation
\graphicspath{{figs/NIPS22_rebuttal_plots/cifar/}}
\begin{figure}[H]\centering
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./bvae/ground_truth.png}
\caption{Ground truth}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{example-image}%{./ae/epoch_200_gen.png}
\caption{AE}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./vae/epoch_200_gen.png}
\caption{VAE (fixed $\gamma$)}
\end{subfigure}     

\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./vaeLG/epoch_200_gen.png}
\caption{VAE (learned $\gamma$)}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./bvae/epoch_200_gen.png}
\caption{$\beta(10)$-VAE}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./waegan/epoch_200_gen.png}
\caption{WAE-GAN}
\end{subfigure}    

\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{example-image}%{./cbvae/5/25/epoch_50_gen.png}
\caption{CBVAE}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{./twostagevae/epoch_last_gen.png}
\caption{2-Stage VAE}
\end{subfigure} \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{example-image}%{./sw/epoch_50_gen.png}
\caption{GoFAE-SW}
\end{subfigure} 

\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{example-image}%{./sf/epoch_50_gen.png}
\caption{GoFAE-SF}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{example-image}%{./cvm/epoch_50_gen.png}
\caption{GoFAE-CVM}
\end{subfigure}     \hfill
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\textwidth]{example-image}%{./ks/epoch_50_gen.png}
\caption{GoFAE-KS} 
\end{subfigure}    
\caption{Comparison of reconstruction between AE, VAE, $\beta$-VAE, WAE-GAN, $2-$Stage VAE and GoFAE.}\label{fig:cifar-recon-imgs}
\end{figure}


% cifar line plots SW and SF
\graphicspath{{figs/NIPS22_rebuttal_plots/cifar/}}
\begin{table}[H]
\captionsetup{type=table} %% tell latex to change to table
\caption{The effects of $\lambda$ with GoFAE-SW (left) and GoFAE-SF (right). From top to bottom, we have: (a) the normality of GoFAE mini-batch encodings using 30 repetitions of Algorithm 1 for different $\lambda$. (b) $p$-value changing from epoch 1-50 under varying $\lambda$. (c) Reconstruction error on the testing set with different $\lambda$. (d) Test statistics value on the testing set with different $\lambda$ }\label{tab:cifar-lines-sw-sf}
\centering
\setlength\tabcolsep{3pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{cM{50mm}M{50mm}}
\toprule
  & GoFAE-SW & GoFAE-SF \\
\midrule
%\rotatebox[origin=c]{90}{plot1} &
(a) & 
\includegraphics[width=14em]{./sw/plots/pval_vs_mi.png} & 
\includegraphics[width=14em]{./sf/plots/pval_vs_mi.png} \\
%\rotatebox[origin=c]{90}{plot2} &
(b) &
\includegraphics[width=14em]{./sw/plots/test_pval_lambda.png} & 
\includegraphics[width=14em]{./sf/plots/test_pval_lambda.png} \\
%\rotatebox[origin=c]{90}{plot3} &
(c) &
\includegraphics[width=14em]{./sw/plots/test_recon_lambda.png} & 
\includegraphics[width=14em]{./sf/plots/test_recon_lambda.png} \\
%\rotatebox[origin=c]{90}{plot4} & 
(d) &
\includegraphics[width=14em]{./sw/plots/test_tstat_lambda.png} & 
\includegraphics[width=14em]{./sf/plots/test_tstat_lambda.png} \\
\bottomrule
\end{tabular}}
\end{table}



% cifarline plots CVM and KS
\graphicspath{{figs/NIPS22_rebuttal_plots/cifar/}}
\begin{table}[H]
\captionsetup{type=table} %% tell latex to change to table
\caption{The effects of $\lambda$ with GoFAE-CVM (left) and GoFAE-KS (right). From top to bottom, we have: (a) the normality of GoFAE mini-batch encodings using 30 repetitions of Algorithm 1 for different $\lambda$. (b) $p$-value changing from epoch 1-50 under varying $\lambda$. (c) Reconstruction error on the testing set with different $\lambda$. (d) Test statistics value on the testing set with different $\lambda$ }\label{tab:cifar-lines-cvm-ks}
\centering
\setlength\tabcolsep{2pt}
\resizebox{\textwidth}{!}{
%\begin{tabular}{l*2{C}@{}}
\begin{tabular}{cM{50mm}M{50mm}}
\toprule
   & CVM & KS \\
\midrule
\rotatebox[origin=c]{90}{plot1} & 
\includegraphics[width=14em]{./cvm/plots/pval_vs_mi.png} & 
\includegraphics[width=14em]{./ks/plots/pval_vs_mi.png} \\
\rotatebox[origin=c]{90}{plot2} & 
\includegraphics[width=14em]{./cvm/plots/test_pval_lambda.png} & 
\includegraphics[width=14em]{./ks/plots/test_pval_lambda.png} \\
\rotatebox[origin=c]{90}{plot3} & 
\includegraphics[width=14em]{./cvm/plots/test_recon_lambda.png} & 
\includegraphics[width=14em]{./ks/plots/test_recon_lambda.png} \\
\rotatebox[origin=c]{90}{plot4} & 
\includegraphics[width=14em]{./cvm/plots/test_tstat_lambda.png} & 
\includegraphics[width=14em]{./ks/plots/test_tstat_lambda.png} \\
\bottomrule
\end{tabular}
}
\end{table}

\fi


==> styles/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

